GeneOH Diffusion: Towards Generalizable Hand-Object Interaction Denoising via Denoising Diffusion

In this work, we tackle the challenging problem of denoising hand-object interactions (HOI). Given an erroneous interaction sequence, the objective is to refine the incorrect hand trajectory to remove interaction artifacts for a perceptually realistic sequence. This challenge involves intricate interaction noise, including unnatural hand poses and incorrect hand-object relations, alongside the necessity for robust generalization to new interactions and diverse noise patterns. We tackle those challenges through a novel approach, GeneOH Diffusion, incorporating two key designs: an innovative contact-centric HOI representation named GeneOH and a new domain-generalizable denoising scheme. The contact-centric representation GeneOH informatively parameterizes the HOI process, facilitating enhanced generalization across various HOI scenarios. The new denoising scheme consists of a canonical denoising model trained to project noisy data samples from a whitened noise space to a clean data manifold and a "denoising via diffusion" strategy which can handle input trajectories with various noise patterns by first diffusing them to align with the whitened noise space and cleaning via the canonical denoiser. Extensive experiments on four benchmarks with significant domain variations demonstrate the superior effectiveness of our method. GeneOH Diffusion also shows promise for various downstream applications. Project website: https://meowuu7.github.io/GeneOH-Diffusion/.

==> articles/exp_tables_old.tex <==
% we need to draw another table with evaluations 
\begin{table}[t]
    \centering
    \caption{ 
    \textbf{Quantitative evaluations and comparisons.} Performance comparisons of our method, baselines, and ablated versions on different test sets using the \textit{first set of evaluation metrics}. \textbf{Bold} numbers for best values and \textit{italic} values for the second best-performed ones.  
    } 
    % \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{@{\;}llccc@{\;}}
        \toprule
        Dataset & Method & \makecell[c]{MPJPE \\ ($mm$, $\downarrow$)} & \makecell[c]{MPVPE \\ ($mm$, $\downarrow$)}  &  \makecell[c]{C-IoU \\  (\%, $\uparrow$)}  \\
        \midrule

        % \multirow{2}{*}{GRAB} & GT & - & - & - & -
        % \\ 
        % \cmidrule(l{17pt}r{17pt}){3-6}

        \multirow{8}{*}{\makecell[c]{GRAB }} & Input & 23.16 & 22.78 & 1.01
        \\ 
        \cmidrule(l{1pt}r{1pt}){3-5}
        
        ~ & TOCH & 12.38 & 12.14  & 23.31
        \\ 

        ~ & TOCH (w/ MixStyle) & 13.36 & 13.03  & 23.70
        \\ 

        ~ & \makecell[l]{Ours (w/o SpatialDiff)} & \textbf{7.83} & \textbf{7.67} & 26.09
        \\ 

        ~ & \makecell[l]{Ours (w/o TemporalDiff)} & \textit{8.27} & \textit{8.13} & \textbf{26.55}
        \\ 

        ~ & \makecell[l]{Ours (w/o Diffusion)} & 8.52 & 8.38 & \textit{26.44}
        \\ 

        ~ & \makecell[l]{Ours (w/o Canon.)} & 10.15 & 10.07 & {24.92}
        \\ 
        
        ~ & \model & {9.28} & 9.22  & {25.27}
        \\ 
        \midrule

        \multirow{6}{*}{\makecell[c]{GRAB \\ (Beta)}} & Input & 17.65 & 17.40  & 13.21
        \\ 
        \cmidrule(l{1pt}r{1pt}){3-5}
        
        ~ & TOCH &  24.10 & 22.90 & 16.32
        \\ 

        ~ & \makecell[l]{TOCH (w/ MixStyle)} & 22.79  & 21.19 & 16.28
        \\ 

        ~ & \makecell[l]{Ours (w/o Diffusion)} & 12.16 & 11.75  & {22.96}
        \\ 

        ~ & \makecell[l]{Ours (w/o Canon.)} & \textit{10.89} & \textit{10.61}  & \textit{24.68}
        \\ 

        ~ & \model & \textbf{9.09} & \textbf{8.98}  & \textbf{26.76}
        \\ 
        \midrule

        \multirow{3}{*}{\makecell[c]{ARCTIC}} & Input & 25.51 & 24.84  & 1.68
        \\ 
        \cmidrule(l{1pt}r{1pt}){3-5}
        
        ~ & TOCH &  14.34 &14.07 & 20.32
        \\ 

        % ~ & \makecell[l]{TOCH (w/ MixStyle)} & -  &-  & -
        % \\ 

        % ~ & \makecell[l]{Ours (w/o Diffusion)} & - & -  & -
        % \\ 

        % ~ & \makecell[l]{Ours (w/o Canon.)} & - & -  & -
        % \\ 

        ~ & \model & 11.57 & 11.09  & 23.49
        \\ 
        \bottomrule
 
    \end{tabular}
    % }
    \label{tb_exp_quant_cmp_ours_toch_toch_metric}
\end{table} 



% we need to draw another table with evaluations 
\begin{table*}[t]
    \centering
    \caption{ 
    % \textbf{Quantitative evaluations and comparisons.} The performance comparisons between our method,  baselines, and ablated models on different test sets regarding the \textit{second set of evaluation metrics}. 
    \textbf{Quantitative evaluations and comparisons.} Performance comparisons of our method, baselines, and ablated versions on different test sets using the \textit{second set of evaluation metrics}. \textbf{Bold} numbers for best values and \textit{italic} values for the second best-performed ones. ``GT'' stands for ``Ground-Truth''. 
    % Quantitative evaluation on the robustness towards novel noisy patterns of our model and baselines. 
    } 
	% \resizebox{\linewidth}{!}{%
    \resizebox{1.0\textwidth}{!}{%
    % \tabcolsep=1pt
    % \begin{tabular}{@{\;}c@{\;}ccccc@{\;}}
\begin{tabular}{@{\;}llcccc@{\;}}
        \toprule
        Dataset & Method & \makecell[c]{IV \\ ($cm^3$, $\downarrow$)} & \makecell[c]{Penetration Depth \\ ($mm$, $\downarrow$)} & \makecell[c]{Proximity Error \\ ($mm$, $\downarrow$)}  &  \makecell[c]{HO Motion Consistency \\  ($mm^2$, $\downarrow$)}  
        % & \makecell[c]{Motion Smoothness \\ ($mm^2$, $\times 10, \downarrow$)}  
        \\
        \midrule

        % \columncolo{yellow}
        \multirow{9}{*}{GRAB} & GT & 0.50 &  1.33 & 0 & 0.51 
        \\ 
        ~ & Input & 4.48 & 5.25 & 13.29 & 881.23 
        \\ 
        \cmidrule(l{15pt}r{17pt}){3-6}
        
        ~ & TOCH & 2.09 & 2.17 & 3.12 & 20.37  
        \\ 

        ~ & TOCH (w/ MixStyle) & 2.28 & 2.62 & 3.10 & 21.29
        \\ 

        ~ & \model (w/o SpatialDiff) & 2.15$\pm$0.02 & 2.29$\pm$0.03 & 6.71$\pm$1.09 & 12.16$\pm$0.67 
        \\

        ~ & \model (w/o TemporalDiff) & \textbf{0.86}$\pm$0.02 & \textbf{1.54}$\pm$0.02 & {3.93}$\pm$0.31 & {9.36}$\pm$0.68  
        \\ 

        ~ & \model (w/o Diffusion) & \textit{1.07} & \textit{1.70} & \textit{2.63}  & 10.05 
        \\ 

        ~ & \model (w/o Canon.) & 1.57$\pm$0.02 & 1.83$\pm$0.03 & 2.91$\pm$0.28  & \textit{1.30}$\pm$0.03 
        \\ 

        ~ & \model & 1.22$\pm$0.01 & 1.72$\pm$0.01 & \textbf{2.44}$\pm$0.18  & \textbf{0.41}$\pm$0.01 
        \\ 
        \midrule

        \multirow{7}{*}{\makecell[c]{GRAB \\ (Beta)}} & GT & 0.50 & 1.33 & 0 & 0.51 
        \\ 
        ~ & Input & 2.19 &  4.77 & 5.83 & 27.58 
        \\
        \cmidrule(l{15pt}r{17pt}){3-6}

        ~ & TOCH & 2.33 &  2.77 & 5.60 & 25.05 
        \\

        ~ & TOCH (w/ MixStyle) & 2.01 &  2.63 & 4.65  & 17.37 
        \\

        ~ & \model (w/o Diffusion) & 1.98 & 2.06 & \textit{3.00}  & 11.99 
        \\ 

        ~ & \model (w/o Canon.) & \textit{1.79}$\pm$0.02 & \textit{1.73}$\pm$0.03 & 3.19$\pm$0.15  & \textit{1.28}$\pm$0.03 
        \\ 

        ~ & \model & \textbf{1.18}$\pm$0.00 & \textbf{1.69}$\pm$0.01 & \textbf{2.78}$\pm$0.14  & \textbf{0.54}$\pm$0.00 
        \\ 
        \midrule

        \multirow{6}{*}{HOI4D} & Input & 2.26 & 2.47 & -  & 46.45 
        \\
        \cmidrule(l{15pt}r{17pt}){3-6}
        
        % \multirow{3}{*}{HOI4D} & TOCH & 4.87 & - & 6.68 & 23.82
        % \\ 

        ~ & TOCH (w/ MixStyle) & 4.31 & 4.96 & - & 25.67 
        \\ 

        ~ & TOCH (w/ Aug.) & 4.20 & 4.51 & -  &  25.85 
        \\ 

        ~ & \model (w/o Diffusion) & 3.16 & 3.83 & -  & 18.65 
        \\ 

        ~ & \model (w/o Canon.) & \textit{2.37}$\pm$0.02 & \textit{3.57}$\pm$0.03 & -  & \textit{12.80}$\pm$0.79 
        \\ 

        ~ & \model & \textbf{1.99}$\pm$0.02 & \textbf{2.14}$\pm$0.02 & -  & \textbf{9.75}$\pm$0.88 
        \\ 
        \midrule

        \multirow{4}{*}{ARCTIC} & GT & 0.33 & 0.92 & 0 & 0.41
        \\
        ~ & Input & 2.28 &  4.89 & 15.21 & 931.69
        \\
        \cmidrule(l{15pt}r{17pt}){3-6}

        ~ & TOCH & - & - & - & -
        \\ 
        % ~ & TOCH (w/ MixStyle) & - & - & - & -
        % \\ 

        % ~ & \model (w/o Diffusion) & - & - & -  & -
        % \\ 

        % ~ & \model (w/o Canon.) & - & - & -  & -
        % \\ 

        ~ & \model & 1.35 $\pm$ 0.01 & 1.91 $\pm$ 0.02  & 2.69 $\pm$ 0.11  & 0.85 $\pm$ 0.00
        \\ 
        
        \bottomrule
 
    \end{tabular}
    }
    % }
    % \vspace{-16pt}
    \label{tb_exp_quant_cmp_ours_toch}
\end{table*} 



==> articles/method_old.tex <==
\section{Generalizable Hand-Object Interaction Denoising via Denoising Diffusion}

% Given a noisy hand-object interaction trajectory with $K$ frames in total and a fixed time interval for each pair of adjacent frames $(\hat{\mathcal{H}}, \mathbf{O})  = \{ (\hat{\mathbf{H}}_k, \mathbf{O}_k) \}_{k=1}^K$ with the noisy hand mesh $\hat{\mathcal{H}}_k$
% and the object mesh $\mathbf{O}_k$ at each frame, we wish to remove noise from the hand trajectory $\hat{\mathcal{H}}$ and output a clean sequence $\mathcal{H}$ free of unrealistic interactions observed in the input sequence. Compared with tracking object poses, tracking hands is more difficult and ill-posed especially those that rely on a few cameras~\cite{zhou2022toch}. Therefore, we assume the object poses are rather accurate and only consider refining hand trajectories for physics-aware interaction sequences. 
% ~\eric{why not denoise the object trajectory? justify this by citing other works or explain that.} The denoised trajectory outght to be natural and human-like free of wired poses or motions, able to interact with the object in a physically plausible way without penetrations or inconsistent motions. The denoising algorithm should be generalizable across objects, various interactions (\emph{e.g.,} moving a camera, opening a scissor), and different noise distributions (\emph{e.g.,} simple Gaussian distributions, rather complex noise caused by inaccurate visual estimations). Designing a generalizable denoising algorithm is very challenging and is an ill-posed problem in nature, considering the ambiguity of the denoising task and the expectation for natural and human-like manipulations. We, therefore, tackle the problem through a data-driven approach. We wish to devise a denoising model that can learn the generalizable denoising strategy from data. By only observing a limited number of interaction data, we wish it able to generalize to unseen objects, novel interactions, and noise. \eric{
% We aim to remove noise from a noisy hand-object interaction trajectory with $K$ frames, denoted as $(\hat{\mathcal{H}}, \mathbf{O}) = { (\hat{\mathbf{H}}_k, \mathbf{O}_k) }{k=1}^K$, where $\hat{\mathcal{H}}_k$ and $\mathbf{O}_k$ represent the noisy hand mesh and object mesh at each frame, respectively. Given that hand poses are more prone to noises due to their high degree of freedom, we refine hand trajectories assuming accurate object poses following previous works~\cite{zhou2022toch,grady2021contactopt,taheri2020grab}. The denoised trajectory should be natural and realistic, faithfully depicting hand-object interaction in a physically plausible manner without penetrations or inconsistent hand and object motions. The problem is ill-posed in nature so previously researchers have turned to data-driven approaches~\cite{zhou2022toch,grady2021contactopt,zhou2021stgae}. However, it remains a challenge how to devise a denoising model that can learn a generalizable denoising strategy from a limited amount of training data and generalize to unseen objects, novel interactions, and different noise patterns. }
We aim to remove noise from a noisy hand-object interaction trajectory with $K$ frames, denoted as $(\hat{\mathcal{H}}, \mathbf{O}) = \{ (\hat{\mathbf{H}}_k, \mathbf{O}_k) \}_{k=1}^K$, where $\hat{\mathbf{H}}_k$ and $\mathbf{O}_k$ represent the noisy hand mesh and object mesh at each frame, respectively. Given that hand poses are more prone to noises due to their high degree of freedom, we refine hand trajectories assuming accurate object poses following previous works~\cite{zhou2022toch,grady2021contactopt,taheri2020grab}. The denoised trajectory should be natural and realistic, faithfully depicting hand object interaction in a physically plausible manner without penetrations or inconsistent hand and object motions. The problem is ill-posed in nature so previously researchers have turned to data-driven approaches~\cite{zhou2022toch,grady2021contactopt,zhou2021stgae}. However, it remains a challenge how to devise a denoising model that can learn a generalizable denoising strategy from a limited amount of training data and generalize to unseen objects, novel interactions, and different noise patterns.

% The core of our method to achieve the generalizable HOI denoising is two key designs. 1) In order to parameterize the interaction sequence faithfully in a physics-aware and generalizable way, we propose our novel and effective HOI representation \rep, generalized contact-centric hand-object spatial and temporal relations. We introduce the concept of generalized contact points to minimize cross object distribution gap. The core for its generalization ability is utilizing such points to normalize the encode hand-object spatial and temporal relations. 2) We devise a denoising strategy by leveraging diffusion models to solve the denoising task to resolve the challening of generalizing to different noise. The key to the generalization is learning how to denoise from a noise sample formed by perturbing data points using a varaiety of noise scales to the data manifold. Our overall framework is depicted in Figure~\ref{fig_method_consist_rep}. In the following text, we will detail our representations and the denoising strategy.

To achieve generalizable HOI denoising, our method revolves around two key designs. Firstly, we propose a novel HOI representation named ``Generalizable generalized contact-centric Hand-Object spatial and temporal relations'', or \rep for short, which accurately represents the interaction sequence in a physics-aware and generalizable manner. The core of \rep is representing and canonicalizing the interaction around the interaction region using generalized contact points and hand-object spatial and temporal relations. This enables cross-object and cross-interaction generalization.
% The core of \rep is representing and canonicalizing the interaction around the interaction region. We introduce generalized contact points to represent objects in a compact and cross-object aligned way and also informative to the interaction. We then propose hand-object  spatial and temporal relations, employing generalized contact points for encoding and canonicalization, to enable cross-object and cross-interaction generalization.
% Secondly, we develop a denoising strategy that leverages diffusion models to tackle the challenge of generalizing to various types of noise. The diffusion model learns how to denoise from the noise space constructed by perturbing data points with varying noise scales. The key aspect of our strategy is leveraging this noise space to align different noise distributions.  By first diffusing the noisy input to the unified noise space and then denoising it, our model can effectively generalize to unseen noise. 
Secondly, we develop a denoising strategy that leverages diffusion models to align different noise distributions and effectively generalize to unseen noise. By diffusing the noisy input to the unified noise space and then denoising it, our model effectively tackles various types of noise.
Our overall framework is depicted in Figure~\ref{fig_method_pipeline}. We will then detail our representations and the denoising strategy in Section~\ref{sec:geneoh} and Section~\ref{sec:diffusion} respectively.

% ~\eric{maybe rename the strategy to highlight the generalizability?}.
% ~\eric{you can briefly describe the magic behind generalizability the both the two core designs after introducing them.}

\begin{figure*}[h]
  \centering
  % \includegraphics[width=1.0\textwidth]{figs/pipeline_10.pdf}
  \includegraphics[width=1.0\textwidth]{figs/pipeline_21.pdf}
  \caption{ 
  \textbf{Generalizable hand-object interaction denoising via denoising diffusion.} Our method comprises two key designs: 1) A generalizable HOI representation \rep, Generalizable generalized contact-centric Hand-Object spatial and temporal relations. It consists of three parts and can represent the HOI in a cross-object, cross-interaction generalizable way. 2) A generalizable hand-object interaction denoising strategy based on diffusion models (\rep Diffusion). We propose a ``denoising via diffusion'' strategy for denoising to enhance noise-level generalization. We further design a cascaded denoising strategy, composed of three denoising stages, to remove noise from the noisy input effectively. For instance, the input noisy trajectory shown in the figure suffers from obvious penetrations, unnatural poses, and missing contacts that are not sufficient to support manipulations. Our hand trajectory denoising module removes such unnatural poses. The spatial denoising module then resolves remaining penetrations. After that, the temporal denoising module addresses other issues such as missing contacts, leading to a realistic manipulation sequence finally. 
  % To effectively clean noise from the input trajectory, we further design a cascaded denoising strategy that removes certain kinds of noise from the observation sequentially.  
  % For instance, in the input noisy trajectory shown in the figure, we observe penetrations, unnatural poses, and missing contacts that are not sufficient to support manipulations. The hand trajectory denoising module removes such unnatural poses and generates a human-like hand trajectory. But the motion-denoised trajectory still suffers from penetrations and missing contacts. Then, the spatial denoising module effectively resolves such penetrations. After that, the temporal denoising module removes unrealistic contacts and other inconsistent hand-object motions for a physically plausible denoised trajectory. 
  % Then, the spatial denoising module 
  % model a large unifed noise space  
  % solve the denoising problem via the ``denoising via diffusion'' approach to 
  % cascaded hand-object interaction denoising strategy leveraging diffusion
  % can generalize well to different noise distributions leveraging diffu
  % leveraging diffusion models for a 
  % for encoding the HOI process\rep: Generalizable generalized contact-centric hand-object spatial and temporal relations
  % We represent the input noisy interaction sequence as several trends of information and denoise them via a diffusion-based cascaded denoising strategy. Each denosing module in the cascaded denoising process focuses on a single part of the representation.
  % \eric{We should show the trajectory in a sequence. Right now the triangle view is quite confusing. Also top left corner, it should be ``input noisy hand trajectory'' and ``input object 6D pose trajectory''. I don't think you need to put generalized contact points to the input. For GeneOH representation, what is canonicalized hand trajectory? maybe we should use semitransparent color to show the object, highlighting their aligned poses. Shouldn't there be some arrows in spatial relation? The spatial relationship and temporal relationship are not very informative. For temporal relationship, I imagine you can at least visualize the relative velocity between a pair of hand-object points. The denoising pipeline, again we should show sequence rather than a triangle. We sould highlight the difference between the three denoised trajectories, either visually or using some text. Right now, the three trajectory does not look different at all. It is no better than not showing the actual trajectory but just use some text descriptions.}
  }
  \label{fig_method_pipeline}
\end{figure*}


\begin{figure}[h]
  \centering
  \includegraphics[width=0.45\textwidth]{figs/reps-2.pdf}
  \caption{ 
  \textbf{Generalized contact-centric hand-object spatial and temporal representations. }
  (\textit{Left (a)}:) Generalized contact points. We calculate the generalized contact points (\textcolor{blue}{blue} points) with normals (\textcolor{pink}{pink} arrows) from the input noisy trajectory. The generalized contact points $\mathbf{P}_k$ at each frame $k$ is associated with a 6D pose  $(\mathbf{R}_k, \mathbf{t}_k)$. 
  % The generalized contact points $\{ \mathbf{P}_k \}$ are the same suit of points across all frames posed by their corresponding 6D pose 
  % The generalized contact points $\mathbf{P}_k$ at each frame $k$ is associated with a 6D pose $(\mathbf{R}_k, \mathbf{t}_k)$. 
  (\textit{Middle (b)}:) Generalized contact-centric hand-object spatial relations. For each object point $\mathbf{o}_k \in \mathbf{P}_k$, the representation contains its position $\mathbf{o}_k$, its normal vector $\mathbf{n}_k$, and the relative position from it to each of the hand keypoint ($\mathbf{h}_k - \mathbf{o}_k$). That information is calculated in the canonicalized frame $k$.
  % where the generalized contact points and the hand keypoints are canonicalized via the 6D pose $(\mathbf{R}_k, \mathbf{t}_k)$ of the generalized contact points. 
  (\textit{Right (c)}:) Generalized contact-centric hand-object temporal relations. For each object point $\mathbf{o}_k \in \mathbf{P}_k$, the representation contains its normal vector $\mathbf{n}_k$, and the relative velocity from it to each of the hand keypoint ($\mathbf{v}_k^{\mathbf{h}} - \mathbf{v}_k^{\mathbf{o}}$). 
  % Those information is calculated in the canonicalized frame $k$, where the generalized contact points and the hand keypoints are canonicalized via the 6D pose $(\mathbf{R}_k, \mathbf{t}_k)$ of the generalized contact points. 
  % The generalized contact points trajectory 
  % Generalized contact points (blue points) with normals (pink vectors) selected from the object based upon their minimum distances to the hand trajectory.  Right (b): Contact-centric hand-object spatial relations. The representation is computed from per-frame hand shape and generalized contact points canonicalized via the orientation and the center of the contact points.\eric{It is not clear what the representation is. Also are the generalized contact points unique for each sequence or each frame? from the figure seems it is for the whole sequence, which is not very intuitive to me why.} 
  }
  \label{fig_method_consist_rep}
\end{figure}

\subsection{\rep: Generalizable Generalized Contact-Centric Hand-Object Spatial and Temporal Relations}
\label{sec:geneoh}
% Designing a HOI denoising model that achieves cross-object and cross-interaction generalizability presents a significant challenge. It involves striking a balance between expressive modeling of objects and interactions, which requires sufficient information, and ensuring generalizability to new objects and interactions. To address this challenge, we focus on developing effective representations for solving the problem. The ideal HOI representation should accurately capture the interaction dynamics, highlight any unusual phenomena like object penetrations, and exhibit robust generalization across different objects and diverse interaction types. To achieve this, we leverage interaction regions to parameterize and normalize the interactions. Although human behaviors can vary significantly when interacting with objects of different shapes, the specific interaction patterns within the interaction region tend to exhibit similarities. For example, while grasping the handle of a mug and the handle of a bucket may involve different global shapes, the localized interaction patterns can be quite similar. This insight gives us the chance to leverage such interaction regions for representing HOI to enhance its generalization ability towards unseen objects and interactions. Based on the fact that the interaction region plays a crucial role in the interactions, we are able to design our generalizable representations without sacrificing its expressiveness. 
 
% Specifically, to effectively represent the HOI process, we comprise our representation by the following three types of information. 
% First, to faithfully represent hand-centric information, we include hand trajectories into the representation. To enhance generalization across objects and interactions, we apply canonicalization techniques to the hand trajectories.   
% Secondly, we adopt an object-centric approach to represent interactions expressively and highlight unnatural interaction phenomena. This object-centric approach allows us to model object constraints, which have a significant influence on hand shapes and kinematic motions during interactions. By designing hand-object spatial relations and hand-object temporal relations, we can effectively capture and describe the hand-object interactions, including unnatural phenomena. 

% The above three types of information, namely the hand trajectory, hand-object spatial relations, and hane-object temporal relations, cconstitute our HOI representation \rep, Generalizable Generalized Contact-Centric Hand-Object Spatial and Temporal Relations. Next, we will detail the representation. 

Designing an HOI denoising model that achieves cross-object and cross-interaction generalizability presents a significant challenge. It involves striking a balance between expressive modeling of objects and interactions and ensuring generalizability to new objects and interactions. To address this challenge, we focus on developing effective representations. The ideal HOI representation should accurately capture the interaction dynamics, highlight any unusual phenomena like geometric penetrations, and exhibit robust generalization across different objects and diverse interaction types.

To achieve this, we leverage interaction regions on the objects to parameterize and normalize the interactions. This will not sacrifice the representation expressivity since interactions are usually localized around the interaction regions. Moreover, such localized interactions tend to exhibit similarities in many different HOI scenarios after a proper global pose normalization, facilitating a cross-object and cross-interaction generalization. For example, while grasping the handle of a mug and the handle of a bucket may involve different global shapes, the localized interaction patterns can be quite similar.

To reflect the above insight, we comprise our representation of three types of information: hand trajectories, hand-object spatial relations, and hand-object temporal relations. The hand trajectories can faithfully represent hand-centric information and we apply a root pose canonicalization technique to further enhance its generalizability across objects and interactions. The hand-object spatial and temporal relations are modeled in a contact-centric way focusing on the localized interaction regions. This allows modeling object constraints to the hand poses and kinematic motions during interactions, helping to reduce unnatural phenomena. The three types of information constitute our HOI representation, named \rep, Generalizable generalized contact-centric Hand-Object spatial and temporal relations. We will then detail the design of \rep.

\noindent\textbf{Generalized contact points.} 
In our representation, the interaction region is grounded on points sampled from the object surface close to the hand trajectory, which we refer to as ``generalized contact points''. To identify these points, we first define a region containing object surface points whose minimum distance to the hand trajectory does not exceed a threshold value of $r_c$, which we set to 5mm. We then sample $N_o$ points denoted as $\mathbf{P}\in \mathbb{R}^{N_o\times 3}$ from this region to serve as the generalized contact points. The sequence of these points across all frames is represented by $\mathcal{P} = \{ \mathbf{P}_k \}_{k=1}^K$, where $\mathbf{P}_k$ represents the points at frame $k$. Each $\mathbf{P}_k$ is associated with a 6D pose, consisting of the object's orientation (or the orientation of the first part for articulated objects), denoted as $\mathbf{R}_k$, and the center of $\mathbf{P}_k$, denoted as $\mathbf{t}_k$. This pose, represented as $(\mathbf{R}_k, \mathbf{t}_k)$, is then used to normalize and encode hand trajectories, as well as hand-object spatial and temporal representations.
% points almost in contact with the hand but may not be necessarily contact points.
% To represent the interaction based on the interaction region, we 
% To effectively model object constraints in the generalizable denoising process, we need to figure out which part of information is both representative for the interaction sequence and also generalizable across different objects and interaction sequences. Based on the observation that we humans may interact with objects, though with disparate global shapes, in similar ways when observed from a local view around the interaction region, such as opening a laptop and opening a car hood. Moreover, object points near the interaction region are much more important to depict the role of the object than those lying far from it. 
% We therefore propose to sample points from the interaction region, which we denote as ``generalized contact points'' (since they are points almost in contact with the hand trajectory but are not necessarily contact points), for representing objects and to encode hand-object interactions, to encourage the cross-object and cross-interaction generalization. 



% \todo{whole hand mesh v.s. keypoints?, bendign fingers? transpose?}

% \todo{and sine we trust the object poses}

\noindent\textbf{Canonicalized hand trajectories.} 
To effectively model hand-centric information~\cite{zhang2021manipnet}, we include hand trajectories in our representation. We discovered that augmenting object-centric HOI representations~\cite{zhou2022toch} with hand-centric information, such as the hand trajectory, effectively improves the ability to model high-frequency hand poses. Relying solely on object-centric representations results in plain and over-smoothed hand poses. To represent the hand, we leverage hand keypoints instead of overall hand meshes, as they offer a compact and expressive representation~\cite{zhang2021manipnet} while preserving high-frequency pose details. We use 21 hand joint points as keypoints and represent the hand trajectory as the sequence of these keypoints, denoted as $\mathcal{J} = \{ \mathbf{J}_k \in \mathbb{R}^{N_h\times 3} \}_{k=1}^K$, where $N_h = 21$ is the number of keypoints.

To further encourage cross-object and cross-interaction generalization ability, we introduce two strategies. Firstly, to mitigate the influence of object poses on the hand trajectory, which can vary significantly across different interactions, we canonicalize the hand trajectories using the poses of the generalized contact points. Specifically, we employ the object's 6D pose $(\mathbf{R}_k, \mathbf{t}_k)$ at each frame $k$ to canonicalize the hand keypoints $\mathbf{J}_k$ at that frame, resulting in a sequence of canonicalized hand keypoints $\bar{\mathcal{J}} = \{\bar{\mathbf{J}}_k\}_{k=1}^K$. The canonicalization operation is defined as $\bar{\mathbf{J}}_k = (\mathbf{J}_k - \mathbf{t}_k) \mathbf{R}_k^T$, where $\mathbf{R}_k^T$ denotes the transposed matrix of $\mathbf{R}_k$. However, even after canonicalization, the alignment of $\bar{\mathcal{J}}$ across different interactions may not be ideal due to variations in the canonicalized object orientations. For example, the canonicalized handle of a bucket may point upwards, while that of a mug may point to the left. To address this issue, we introduce the second strategy: train-time random rotation augmentation. This augmentation applies a single random rotation matrix to the whole canonicalized hand trajectories and serves as a training strategy to enhance generalization, but is not included in the \rep representation. We will simply use $\bar{\mathcal{J}}$ to denote the canonicalized hand trajectory in our representation.
% We include hand trajectories in our representation considering their effectiveness in modeling hand-centric information~\cite{zhang2021manipnet}.  In our early experiments, we discover that simply augmenting an object-centric HOI representation~\cite{zhou2022toch} with hand-centric information such as the hand trajectory can effectively improve the ability in modeling high-frequency hand poses. By contrast, only relying on object-centric representations would result in plain and over-smoothed hand poses. 
% Instead of using the overall hand meshes, which contain redundant information and are not friendly for networks, we choose to leverage hand keypoints to represent the hand. Hand keypoints offer a compact and expressive representation of hands~\cite{zhang2021manipnet}, while preserving high-frequency pose details like finger bending. Specifically, we use 21 hand joint points as keypoints.  The hand trajectory is represented as the sequence of these keypoints, denoted as $\mathcal{J} = \{ \mathbf{J}_k \in \mathbb{R}^{N_h\times 3} \}_{k=1}^K$, where $N_h = 21$ is the number of keypoints. To further encourage the cross-interaction generalization ability of the representation, we introduce two strategies. Firstly, to mitigate the influence of object poses on the hand trajectory, which can vary significantly across different interactions, we canonicalize the hand trajectories using the poses of the generalized contact points. Specifically, we employ the object's 6D pose $(\mathbf{R}_k, \mathbf{t}_k)$ at each frame $k$ to canonicalize the hand keypoints $\mathbf{J}_k$ at that frame, resulting in a sequence of canonicalized hand keypoints $\bar{\mathcal{J}} = \{\bar{\mathbf{J}}_k\}_{k=1}^K$. The canonicalization operation is defined as $\bar{\mathbf{J}}_k = (\mathbf{J}_k - \mathbf{t}_k) \mathbf{R}_k^T$, where $\mathbf{R}_k^T$ denotes the transposed matrix of $\mathbf{R}_k$. Even after canonicalization, the alignment of $\bar{\mathcal{J}}$ across different interactions may not be ideal due to variations in the canonicalized object orientations. For example, the canonicalized handle of a bucket may point upwards, while that of a mug may point to the left. To address this, we introduce a random rotation augmentation during training. This augmentation applies a random rotation matrix to the canonicalized hand trajectories. It serves as a training strategy to enhance generalization and is not included in the final representation. 

% The  canonicalized hand trajectory $\bar{\mathcal{J}}$  in our representation is defined as: 
% \begin{equation}
%     \bar{\mathcal{J}} = \{ \bar{\mathbf{J}}_k \}_{k=1}^K. 
% \end{equation}
% $\bar{\mathbf{J}}_k$ represents the canonicalized hand keypoints at frame $k$.

% First, to remove the effect of object poses on the hand trajectory, which always vary a lot across different interactions, we canonicalize hand trajectories via  poses of the generalized contact points. Specifically, we use object 6D pose  $(\mathbf{R}_k, \mathbf{t}_k)$  at each frame $k$ to canonicalize the hand keypoints at that frame $\mathbf{J}_k$. We denote the canonicalized hand keypoints as $\bar{\mathbf{J}}_k$. The canonicalization operation is $\bar{\mathbf{J}}_k = (\mathbf{J}_k - \mathbf{t}_k) \mathbf{R}_k^T$, where $\mathbf{R}_k^T$ is the transpose of $\mathbf{R}_k$. After such canoncialization, we still cannot align $\bar{\mathcal{J}}$ very well across different interactions due to the difference between their canonicalized object orientations. For instance, the canonicalized handle of the bucket may points up while that of the mug points to the left. Therefore, we add an random rotation augmentation operation during the training time. It further applies a random rotation matrix to the canonicalized hand trajectories. We regard it as a training trick and spare it in the representation.  
% The canoncialized hand trajectory representation $\mathcal{J}$ is represented as, 
% \begin{equation}
%     \bar{\mathcal{J}} = \{ \bar{\mathbf{J}}_k \}_{k=1}^K. 
% \end{equation}

% Although hand trajectories do not consider object information such as object shape, they are still affected by the interactions with the object. The object pose may change during the interaction. The pose of the hand wrist would also change accordingly. Since the object trajectory may vary a lot across different interaction sequences. The hand trajectories directly taken from each interaction sequence would also be distinct from each other. Therefore, we propose a simple yet effective strategy, canonicalization, to align hand trajectories. 
% \ericg{this is very plain. when writing the method section, the important thing is to explain not only what and how you do, but also why. I don't see why introducing hand representation like this is better than alternatives like TOCH. I don't even know what information needs to be encoded in the HOI representation. A more clear way to organize the whole method section is to explain what information needs to be encoded during HOI first, and then how to make them generalizable.}

% As a detail, since we use generalized contact points $\mathbf{P}_k$ to represent the object for each frame $k$, the object pose used for canonicalization is the 6D pose of $\mathbf{P}_k$. The orientation $\mathbf{R}_k$ is the same to that of the whole object, while the translation $\mathbf{t}_k$ is the center of $\mathbf{P}_k$. 

% Hand trajectories are important for denoising hand-centric information~\cite{zhang2021manipnet}.  
% In our early experiments, we discover that simply augmenting an object-centric representation with the hand-centric information such as the hand trajectory can effectively improve the ability in modeling hands such as high-frequency hand poses. By contrast, simply relying on object-centric representations would result in plain and over-smoothed hand poses. Therefore, to expressively represent the interaction process on the hand aspect, we include hand trajectories into our representation. 

% \todo{other literatures on the object-centric representations}
\noindent\textbf{Generalized contact-centric hand-object spatial relations.} 
To effectively model hand-object spatial relations and highlight unnatural phenomena in a cross-object and cross-interaction generalizable way, we propose a generalized contact-centric hand-object spatial representation. This representation encodes the spatial relations between the hand and the object. We still adopt the hand keypoints and generalized contact points to inherit their merits in compactness and generalization. For each object point $\mathbf{o}_k$ belonging to the generalized contact points $\mathbf{o}_k \in \mathbf{P}_k$, we define the representation as a set of informative statistics. These statistics include the relative offset from the object point to each hand keypoint $\mathbf{h}_k \in \mathbf{J}_k$, \emph{i.e.,} $\{ \mathbf{h}_k - \mathbf{o}_k | \mathbf{h}_k \in \mathbf{J}_k \}$, the object normal $\mathbf{n}_k$ at the point $\mathbf{o}_k$, and the position $\mathbf{o}_k$ of the point itself. These statistics can capture the spatial relationship between the hand and the object and provide valuable information to identify errors.

To encourage generalization across different interactions, we further canonicalize the statistics using the 6D pose of the generalized contact points $(\mathbf{R}_k, \mathbf{t}_k)$. During training, we also apply the same random rotation matrix used for augmenting the hand trajectory to the statistics. 
Formally, we denote the representation centered at the object point $\mathbf{o}_k$ as $\mathbf{s}_k^{\mathbf{o}}$, which is defined as: 
\begin{equation}
\mathbf{s}_k^\mathbf{o} = ((\mathbf{o}_k - \mathbf{t}_k)\mathbf{R}_k^T, \mathbf{n}_k\mathbf{R}_k^T, \{ (\mathbf{h}_k - \mathbf{o}_k)\mathbf{R}_k^T | \mathbf{h}_k \in \mathbf{J}_k\} ). 
\end{equation}
The final representation for hand-object spatial relations is formed by combining $\mathbf{s}_k^\mathbf{o}$ for each object point $\mathbf{o}_k$ belonging to the generalized contact points $\mathbf{P}_k$ across all frames. We represent the spatial relations as $\mathcal{S}$, which is defined as:
\begin{equation}
\mathcal{S} = \{ \{ \mathbf{s}_k^\mathbf{o} | \mathbf{o}_k \in \mathbf{P}_k\} \}_{k=1}^K.
\end{equation}

The above hand-object spatial relations $\mathcal{S}$ could generalize well across objects and interactions as it leverages generalized contact points for representation and canonicalization. This contact-centric view also allows $\mathcal{S}$ to reveal unnatural HOI such as when geometric penetration happens.  


\noindent\textbf{Generalized contact-centric hand-object temporal relations.} 
To complete the denoising task, relying solely on canonicalized hand trajectories and hand-object spatial relations is insufficient, as they do not highlight temporal interaction noise.  Considering an example when the hand moves in the opposite direction to the object motion without touching the object, resulting in a totally wrong interaction sequence without any correct contacts to support the object motion or consistent hand-object motions. Such noise can not be easily detected from hand poses alone since the hand motion itself could be smooth and natural, nor from the hand-object spatial relations since no penetration exists. Therefore, we need to devise representations that encode hand-object temporal relations and reveal temporal noise, such as incorrect contacts that cannot support manipulations and inconsistent hand-object motions. Our key idea is to represent the relative motion between the hand and the object beyond their relative poses. Specifically, to ensure generalizability across objects and interactions, we again take hand keypoints $\mathbf{h}$ to represent hand shape and generalized contact points $\mathbf{o}$ for the object shape, devising the representation in an object-centric manner to effectively model the role of the object. To encode hand-object temporal relations and highlight temporal noise, we consider encoding the relative velocity between each object point $\mathbf{o}_k$ and each hand keypoint $\mathbf{h}_k$ at frame $k$ ($\mathbf{v}_k^{\mathbf{h} \mathbf{o}} = \mathbf{v}_k^{\mathbf{h}} - \mathbf{v}_k^{\mathbf{o}}$), the Euclidean distance between each pair of points ($d_k^{\mathbf{ho}} = \Vert \mathbf{h}_k - \mathbf{o}_k \Vert_2$), and the object velocity $\mathbf{v}_k^o$ in the representation. Jointly considering the statistics of all hand-object point pairs can successfully reveal the temporal noise.
% \todo{xxx need to give examples here?}


To promote generalization across interactions and highlight temporal errors, we decompose the relative velocity $\mathbf{v}_k^{\mathbf{h} \mathbf{o}}$ between each hand point $\mathbf{h}_k$ and object point $\mathbf{o}_k$ into two statistics: $\mathbf{v}_{k,\perp}^{\mathbf{h} \mathbf{o}}$, vertical to the object tangent plane and parallel to the object point normal, and $\mathbf{v}_{k,\parallel}^{\mathbf{h} \mathbf{o}}$, lying in the object's tangent plane. This decomposition enables the model to learn different denoising strategies for the two types of relative velocities and enhance cross-interaction generalization by factoring out object poses.
However, relying solely on relative velocities is insufficient to reveal motion noise in hand-object interactions. The same relative velocity parallel to the normal direction can correspond to a clean state when the hand is far from the object, but a noisy state when they are in contact. To address this, we encode the distance between each hand-object pair and their relative velocities into two statistics, $\{ ( e_{k, \perp}^{ho}, e_{k, \parallel}^{ho} ) \}$, using the following formulation:
\begin{align}
    e_{k, \perp}^{\mathbf{ho}} &= e^{-k\cdot d_{k}^{\mathbf{ho}}} k_b\Vert \mathbf{v}_{k,\perp}^{\mathbf{h} \mathbf{o}}  \Vert_2  \\
    e_{k, \parallel}^{\mathbf{ho}} &= e^{-k\cdot d_{k}^{\mathbf{ho}}} k_a\Vert \mathbf{v}_{k,\parallel}^{\mathbf{h} \mathbf{o}} \Vert_2. 
    % e_{k, \perp}^{\mathbf{ho}} &= e^{-k\cdot d_{k}^{\mathbf{ho}}} k_b\Vert \mathbf{v}_{k,\perp}^{\mathbf{h} \mathbf{o}}  \Vert_2,  
\end{align}
Here, $k$, $k_a$, and $k_b$ are positive hyperparameters, and the term $e^{-k\cdot d_{k}^{\mathbf{ho}}}$ is inversely related to the distance between the hand and object points. This formula allows the statistics for closely located points to be emphasized in the representation.

% Further, to encourage the generalization ability across different interactions and for the purpose of emphasizing errors, we encode the relative velocity $\mathbf{v}_k^{\mathbf{h} \mathbf{o}}$ between each hand point $\mathbf{h}_k$ and the object point $\mathbf{o}_k$ into two statistics in the local object frame.
% Specifically, we decompose $\mathbf{v}_k^{\mathbf{h} \mathbf{o}}$ into two vectors, \emph{i.e.,} $\mathbf{v}_{k,\parallel}^{\mathbf{h} \mathbf{o}}$ that is parallel to the object normal, and $\mathbf{v}_{k,\perp}^{\mathbf{h} \mathbf{o}}$ that lies in the tangent plane of the object point. Such decomposition can factorize out object poses and therefore help increase the cross-interaction generalization ability. Besides, such decomposition could also let the model learn different denoising strategies for two kinds of relative velocities. When the hand point $\mathbf{h}_k$ is moving close to the object point $\mathbf{o}_k$, the hand point should not penetrate the object so that their relative velocity parallel to the normal should be penalized, while another velocity should not be restricted since the hand can slide on the object surface. 
% Given the decomposed relative velocities, we need further consider how to reveal noise existed in hand-object motions. Simply relying on relative velocities is not sufficient. A same relative velocity parallel to the normal direction may correspond to a clean state when hand is far from the object, while a noisy state when they are in contact. Therefore, we further encode the distance between each hand-object pair and their relative velocities into two statistics, $\{ ( e_{k, \parallel}^{ho}, e_{k, \perp}^{ho} ) \}$ via
% \begin{align}
%     e_{k, \parallel}^{\mathbf{ho}} &= e^{-k\cdot d_{k}^{\mathbf{ho}}} k_a\Vert \mathbf{v}_{k,\parallel}^{\mathbf{h} \mathbf{o}} \Vert_2 \\ 
%     e_{k, \perp}^{\mathbf{ho}} &= e^{-k\cdot d_{k}^{\mathbf{ho}}} k_b\Vert \mathbf{v}_{k,\perp}^{\mathbf{h} \mathbf{o}}  \Vert_2,  
% \end{align}
% where $k$, $k_a$ and $k_b$ are hyper-parameters. The parameter $e^{-k\cdot d_{k}^{\mathbf{ho}}}$ is negatively related to hand-object point distance so that the corresponding statistics for points close to each other can be emphasized. 

Then we represent the hand-object temporal motion relations by combining the above statistics for each hand-object point pair across all frames together.  This representation, denoted as $\mathcal{T}$, is defined as follows:
\begin{equation}
    \mathcal{T} = \{ \{  \mathbf{v}_k^\mathbf{o}, \{ d_k^{\mathbf{ho}}, e_{k, \parallel}^{\mathbf{ho}},  e_{k, \perp}^{\mathbf{ho}}  \vert \mathbf{h}_k \in \mathbf{J}_k \} \} \vert \mathbf{o}_k \in \mathbf{P}_k  \}_{k=1}^{K-1}. 
\end{equation}

\noindent \textbf{The \rep representation.} The overall representation, \rep, comprises three components: the canonicalized hand trajectory $\bar{\mathcal{J}}$, the hand-object spatial relations $\mathcal{S}$, and the hand-object temporal motion relations $\mathcal{T}$. Formally, it is represented as:

\begin{equation}
\text{\rep} = \{ \bar{\mathcal{J}}, \mathcal{S}, \mathcal{T} \}.
\end{equation}

% \rep offers several advantages in representing hand-object interactions. It combines hand-centric and object-centric representations, capturing both spatial and temporal aspects of the interaction. Furthermore, \rep effectively reveals and emphasizes unnatural interaction phenomena in both spatial and temporal dimensions. Its design based on generalized contact points-centric encoding and canonicalization ensures strong generalization across different objects and interactions.

% Compared to prior works, 
\rep can be applied to interaction sequences involving rigid or articulated objects. It is expressive, accurately encoding information related to hand-object interactions. Besides, it can highlight spatial and temporal interaction errors. The above advantages make \rep well-suited for the HOI denoising task. 

Regarding prior works, the representation in TOCH~\cite{zhou2022toch}, which expands the concept of contacts to the ambient space, is restricted. It cannot represent the interaction in some cases. Besides, it often struggles with modeling hand shape details. The representation introduced in~\cite{zhang2021manipnet} then encodes the interaction process in a solely hand-centric way. This strategy leads to their limitation in effectively modeling object constraints. 
% They are not very effective in modeling object constraints. 

% TOCH~\cite{zhou2022toch} 
% would fail to represent the interaction when no object normal can reach the hand surface. It often struggles with modeling hand shape details as well. 
% cannot be defined on any interaction state 
% hand-object interactions
% In comparison, TOCH~\cite{zhou2022toch} 
% addressing the issue of incomplete definition present in TOCH~\cite{zhou2022toch} representation~\eric{what is incomplete definition? this is not clear.}. It is expressive, accurately encoding hand-object interactions and handling high-frequency hand poses.~\eric{which is usually an issue for ...} Besides, \rep compactly encodes interaction information in a contact-centric manner, resulting in more effective modeling of object constraints compared to hand-centric representations alone~\cite{zhang2021manipnet}. 

\begin{figure}[h]
  \centering
  \includegraphics[width=0.45\textwidth]{figs/denoising_via_diffusion_v3.pdf}
  \caption{ \textbf{Denoising via diffusion.} The input noisy trajectory is diffused by $t_\text{diff}$ diffusion steps. Then, the perturbed noisy trajectory is cleaned leveraging the denoising process of the diffusion model. 
  }
  \label{fig_method_denoising_after_diffusion}
\end{figure}

\subsection{
% \rep Diffusion: Generalizable Hand-Object Interaction Denoising via Cascaded Denoising Diffusion
\rep Diffusion %: Denoising via Cascaded Denoising Diffusion
% Cascaded Hand-Object Interaction Denoising via Diffusion
} 
\label{sec:diffusion}
% \eric{What is the challenge? The key idea to achieve generalizability?}
% Based upon the above representations, we then denoise the interaction sequence via denoising \rep representations. We leverage diffusion models to realize generalizale denoising.~\eric{why this can be possible? no intuition at all} Basically, we first train diffusion models to learn the denoising strategy from noise from a large noise space composed by perturbing data points by noise with a variety of noise scales. ~\eric{what does this mean? denoising strategy?} The noise space modeled in the diffusion model can naturally bridge the gap between different noise distributions. We further take a denoising after diffusion approach~\ref{fig_method_denoising_after_diffusion} to denoise input noisy data.~\eric{the diffusion approach here means adding noise?}
% It first perturbs noisy inputs by a certain number of timesteps and then denoises the perturbed data so that the distribution gap can be further bridged taking advantage of the forward diffusion steps.~\eric{the denoise step should not appear before ``so that'' since it does not bridge the distribution gap} Therefore, based upon the above design for noise space alignment~\eric{the term suddenly appears. should rigorously name a process first before referring to it.}, the denoising strategy can gracefully generalize across novel noise.~\eric{this is too absolute. need to discuss the generalization regarding noise patterns in depth} 
% \rep with good properties like expressiveness, highlighting errors, and generalization ability across unseen objects and interactions is possible to serve as intermediates for denoising. We can devise many denoising models designed based on the representations for HOI denoising. Considering its generalization ability, the denoising model is expected generalizable at the object level and the interaction level. However, we are further challenged by noise patterns that may vary a lot across different interaction sequences. For instance, in some sequences, the hand trajectory is noisy, lacking smoothness, but only wandering around the object without touching it during the interaction process. However, in some sequences, the hand trajectory is smooth, but frequently penetrates the object. Besides, we usually cannot predict the noise pattern that a denoising model needs to deal with in the real application scenario. Relying on such noisy data to teach a model how to clean them is also not that possible due to the lack of paired ground-truth data. Commonly, a denoising model can only rely on clean data to learn how to denoise. Previous works rely on paired noisy-clean data to solve the problem. They teach the model to convert the noisy data to the clean one. However, they would suffer from the overfitting issue and can hardly generalize to novel noise. Augmenting noisy patterns for training is still not a good solution considering the novel, difficult, unpredictable noise pattern that we may encounter at the test time. Solving this problem requires us to devise a denoising strategy that can handle various kinds of noise. Our approach is first aligning noisy input to a common noise space and then letting the model denoise from this noise space. 
% letting the model to denoise simialr noise. Sp
% Therefore, instead of following prior approaches, we turn to find another trend of denoising strategy that first convert noisy data to a unified noise space and then denoises it. 
% due to complex noise patterns that may vary a lot from each other. 
% solve the problem by teaching the model to denoise noisy data perturbed by adding hand-crafted noise to the clean data
% A denoising model would frequently e
% Based upon \rep with good properties like expressiveness, highlighting errors, and generalization ability across unseen objects and interactions, 
% we can remove noise from the representations to denoise the interaction sequence. However, though we are equipped with \rep with high expressiveness to serve as intermediates for denoising where we can devise many strategies, and also with strong cross-object and cross-interaction generalization ability to prevent the denoising model from overfitting to  spurious cues for denoising, it is still challenging to devise a denoissing model generalizable to novel noise distributions. Solving the denoising problem requires the model to learn how to map noisy data to the clean data. However, common HOI denoising models that learn how to map noisy data with certain noise patterns to the clean data would tend to overfit to noise patterns used for training. Therefore, they are not the most ideal solutions. Augmenting noisy patterns for training is still not a good solution due to complex noise patterns that may vary a lot from each other. It is hard to arrive at a generic solution for various unseen noise. Therefore, we turn to find another trend of denoising model that first convert noisy data to a unified noise space and then denoises it. 

% \todo{add refs}

% Diffusion models~\cite{rombach2022high,ho2020denoising}, a family of generative models, then give us the opportunity to realize the above denoising strategy. As a generative model, diffusion models connect the data manifold and the standard noise distribution. As score-based generative models~\cite{song2019generative,song2020score}, they also learn the mapping from a noise space containing noisy data perturbed via noise of a variety of scales to the manifold. Aligning noisy input to such as noise space and the denoising from it then make it possible to make the denoiesd result with both realism and enough relevance to the noisy input. Specifically, we first perturbs the input noisy data via noise of a certain level. Then we let the diffusion model, trained for this type of data, remove noise from the perturbed noisy data. We term the above denoising strategy as ``Denoising via Diffusion''. The general algorithm is illustrated in  Algorithm~\ref{algo_denoising_via_diffusion}.  Given a noisy input $\hat{x}$, the diffusion model first diffuse the data for $t_\text{diff}$ diffusion steps to move it to the noise space of the diffusion model. Then it denoise the diffused data leveraging the learned denoising function. 

While \rep exhibits generalization ability at the object and interaction levels, designing a generalizable denoising model remains challenging due to varying noise patterns. Noise in interaction sequences may exhibit different patterns, such as noisy hand trajectories lacking smoothness, or frequent hand-object penetrations despite smooth trajectories, which could differ significantly from that observed in the training set. Previous approaches mostly learn a deterministic mapping from noisy to clean sequences based on a specific training set, struggling to generalize to novel noise patterns and suffering from overfitting. Augmenting noisy patterns during training is also ineffective in addressing unpredictable noise encountered during testing.

To address the above challenges, we propose aligning the noise space for the denoising model by converting noisy data into a unified noise space that can bridge different noise distributions. Notice the alignment operation also needs to preserve the identity of the noisy data rather than transforming it into an unrelated noise point. Diffusion models~\cite{rombach2022high,ho2020denoising,dhariwal2021diffusion}, a family of generative models, offer an opportunity to realize this aligning and denoising strategy. Diffusion models have a forward diffusion process that progressively adds noises to input data samples so that they are gradually closer to a standard prior noise distribution. In the other direction, diffusion models also learn backward denoising functions to recover clean samples from the noise space. This forward diffusion and backward denoising exactly match our goal for aligning and denoising respectively. We can similarly diffuse the input noisy HOI representation first and then apply a trained diffusion model to remove the noise.
% As generative models, diffusion models connect the data manifold with a standard noise distribution. Besides, they learn the mapping from a noise space containing noisy data perturbed by noise of various scales to the manifold. Aligning noisy input to such a noise space and denoising from it allows for realistic and relevant denoised results. 
And we term this denoising strategy ``Denoising via Diffusion''. 
In particular, given noisy input $\hat{x}$, the diffusion model applies $t_\text{diff}$ diffusion steps to move the data to the noise space and then denoises the diffused data using the learned denoising function as shown in Algorithm~\ref{algo_denoising_via_diffusion}.
% The general algorithm involves perturbing the input noisy data with a certain level of noise and using the trained diffusion model to remove the noise from the perturbed data.
% Given a noisy input $\hat{x}$, the diffusion model applies $t_\text{diff}$ diffusion steps to move the data to the noise space of the model. Subsequently, it denoises the diffused data using the learned denoising function. 
% The proposed algorithm is outlined in Algorithm~\ref{algo_denoising_via_diffusion}
% adds noise on it to move it to the noise space of the diffusion model by diffusing the data for $t_\text{diff}$ steps. Then, it denoises the perturbed data utilizing the learned denoising function. 
% Such a noise space then make it possible to make the denoised result both with enough realism and also faithfulness to input noisy trajectory. Specifically, we 
% formed by noisy data perturbed 
% whiten by perturbing data via noise of a variety of scales to the data manifold. The perturbed data space is able to serve as the unified noise space that can be utilized to align various noise distributions. By perturbing input noisy data via noise of a certai level, we can align the input to the perturbed data space. Then, the diffusion model removes noise from the perturbed data for cleaning. The process of the above denoising strategy, termed as ``Denoising via Diffusion'' is illustrated in Algorithm~\ref{algo_denoising_via_diffusion}.  The diffusion model first adds noise on the input noisy data $\hat{x}$ to align it to the perturbed data space by diffusing the data for $t_\text{diff}$ steps. Then, it denoises the perturbed data utilizing the learned denoising function. 
% Solving this issue requires us to find a proper way 
% To address this issue, we need 
% generalizable solutions
% suffer from the overfitting issue 
% due to the difficulty in achieving the generalization ability to novel noise distributions.  
% A trivial denoising model that learns how to map the noisy data with certain noise patterns would suffer from the overfitting issue and can hardly generalize to novel noise. To address this issue, the key to our solution is leveraging diffusion models to solve the denoising problem. 

% The intuition is that the denoising process learned by the diffusion model presents us with the opportunity align different noise distributions. It learns how to project data points perturbed by uniform standard noise with different noise scales to the data manifold. Therefore, given a noisy data point with an arbitrary noise pattern, we can use the diffusion process to align it to the noise space depicted by the diffusion model. We can complete the denoising task by projecting the perturbed noisy data back to the data manifold. 

% With the expressiveness and the generalization ability of \rep, as well as the above denoising strategy, a possibility to accomplish the generalizable denoising task is treating \rep as an intermediates for denoising and remove noise from it. However, it is still very challening to clean the representation all at once. \rep contains three types of information, \emph{i.e.,}, canonicalized hand trajectories $\bar{\mathcal{J}}$, hand-object spatial relations $\mathcal{S}$, and the hand-object temporal motion relations $\mathcal{T}$. Designing an effective diffusion model for \rep is not an easy thing. For instance, just designing effective networks for such representations, like encoding network, denoising network, has no clear answer from the literature and requires us to innovate new architectures. Therefore, instead of using a single denoising network to clean the entire representation, we propose a cascaded denoising strategy that denoises each type of information sequentially. Each denoising stage operates on the output of the previous stage. Specifically, we train three diffusion models, each for $\bar{\mathcal{J}}$, $\mathcal{S}$, and $\mathcal{T}$ respectively. Each of them is trained by their corresponding representations of clean data sequences from a MoCap dataset for training. Each diffusion model is then easy to design by adapting existing model architectures. 
% Given a noisy input, the cascaded denoising model cleans the each part of the representation sequentially. Specifically, the cascaded denoising is composed of 
% 1) hand motion denoising via diffusion, where we denoise the noisy hand trajectory $\hat{\mathcal{J}}$ without considering object constraints; 
% 2) hand-object spatial denoising via diffusion, where we denoise the noisy spatial representations $\hat{\mathcal{S}}$ to resolve incorrect spatial interaction phenomena such as penetrations, and 
% % $\mathcal{S}$ to resolve incorrect spatial interaction phenomena such as penetrations, and 
% 3) hand-object temporal denoising via diffusion, where we denoise the hand-object temporal motion relation representation $\hat{\mathcal{T}}$ to induce correct contact and encourage consistent hand-object motions. 

Applying the above denoising strategy on \rep seems a promising solution for generalizable denoising. However, designing an effective diffusion model for \rep is challenging due to the three distinct types of information it contains: canonicalized hand trajectories $\bar{\mathcal{J}}$, hand-object spatial relations $\mathcal{S}$, and hand-object temporal motion relations $\mathcal{T}$. To address this, we propose a cascaded denoising strategy that sequentially denoises each type of information, building upon the output of the previous stage. Specifically, we train three diffusion models for $\bar{\mathcal{J}}$, $\mathcal{S}$, and $\mathcal{T}$ respectively, on clean data sequences from a MoCap dataset. Given a noisy input, the cascaded denoising model sequentially deploys the three diffusion models to: 1) clean the canonicalized hand trajectories without considering object constraints; 2) denoise hand-object spatial relations to address incorrect spatial artifacts such as penetrations; 3) refine hand-object temporal motion relations to promote correct contact and consistent hand-object motions.

% With the expressiveness and the generalization ability of \rep, as well as the above denoising strategy, a potential solution for achieving generalizable denoising is cleaning the noisy interaction sequence by cleaning noisy representations of it. However, it is still very challenging for us to devise an effective denoising model. With three distinct types of information in \rep, that is canonicalized hand trajectories $\bar{\mathcal{J}}$, hand-object spatial relations $\mathcal{S}$, and hand-object temporal motion relations $\mathcal{T}$, designing an effective diffusion model for it is not an easy thing. Even an encoder-decoder like network may require our special innovations. To address this, we propose a cascaded denoising strategy that sequentially denoises each type of information. Each denoising stage builds upon the output of the previous stage. Specifically, we train three diffusion models: one for $\bar{\mathcal{J}}$, one for $\mathcal{S}$, and one for $\mathcal{T}$. These models are trained on corresponding representations of clean data sequences from a MoCap dataset. By adapting existing model architectures, the design of each diffusion model becomes rather easy. Given a noisy input, the cascaded denoising model sequentially cleans each part of the representation via the following three stages: 1) hand motion denoising via diffusion, focusing on the noisy hand trajectory $\hat{\mathcal{J}}$ without considering object constraints; 2) hand-object spatial relations denoising via diffusion, targeting the noisy spatial representations $\hat{\mathcal{S}}$ to address incorrect spatial interaction phenomena, such as penetrations, and 3) hand-object temporal motion relations denoising via diffusion, aiming to clean the representation $\hat{\mathcal{T}}$ and promote correct contact and consistent hand-object motions.


% cleans each separate part of the representation sequentially. Specifically, we train a diffusion model for each type of representation individually
% three diffusion models for 
% three types of information separately hand trajectories $\mathcal{J}$, hand-object spatial relations $\mathcal{S}$, and 
% that sequentially cleans each part of the representation
% It requires us to devise effective networks for such representations, like the encoding network, denoising network, \emph{etc.}. Des
% Designing an effective diffusion model for \rep is 
% It is hard to design a diffusion model for the entire representation with three different types of information. 
% Therefore, we learn three separate diffusion models for each part of the representation. And we devise a cascaded denoising strategy that applies those diffusion models to clean their corresponding representations sequentially. 
% Specifically, the cascaded denoising is composed of 
% 1) hand motion denoising, where we denoise hand trajectories $\{ \mathbf{J}_k \}_{k=1}^K$ with no consideration on object constraints, 2) hand-object spatial denoising, where we denoise the generalized contact-centric hand-object spatial relations to resolve incorrect spatial interaction phenomena such as penetrations, and 3) hand-object temporal denoising, where we denoise the hand-object temporal motion relation representation to induce correct contact and encourage consistent hand-object motions.
% ~\eric{should explain why leveraging a three-stage diffusion. talk about its advantages and comparison with alternatives.}
% At the training time, for each denoising module, we train a diffusion model for its corresponding part of representations based upon ground-truth interaction sequences from the training dataset. When leveraging the diffusion model for sampling, we adopt a denoising after diffusion approach~\ref{fig_method_denoising_after_diffusion}.
% ~\eric{what does this mean? not clear} 
% It first diffuse the representation for a certain number of timesteps. Then the denoising function learned by the diffusion model operates on the diffused representations for denoising. 

% Specifically, we learn three diffusion models for each part of \rep, that is a hand motion diffusion model for hand trajectories $\mathcal{J}$, a hand-object spatial diffusion model for spatial relations $\mathcal{S}$, and a hand-object temporal diffusion model for temporal motion relations $\mathcal{T}$. Then, we denoise the input trajectory via three denoising stages, that is hand motion denoising (MotionDiff), hand-object spatial denoising (SpatialDiff), and hand-object temporal denoising (TemporalDiff). We will detail on each denoising stage in the following text. 
% Based upon the expressive and generalizable \rep representations and the above denoising philosophy, we present a cascaded hand-object denoising strategies leveraging diffusion models. 

% We then design a denoising leveraging diffusion models and 
% can hardly generalize to novel noise 
% from a restricted noise distribution to clean data would very likely overfit to certain noise patterns, failing to generalize to data with novel noise. 
% The key to address this issue for a generalizable denoising model in a most straightforward yet most effective way is learning a rather universal denoiser that can map noise from a vast space to the data manifold. The secondary key is align the observed noisy data to the noise space modeled by the denoiser via perturbations. We then leverage diffusion models to realize them. Diffusion models as a family of generative models learn how to project a noise point from a standard Normal distribution to the data manifold~\cite{ho2020denoising,rombach2022high}. Instead of xxx, it learns how to project data points perturbed by noise with different scales to the data point. Our key design is learning how to denoise \rep representations from a large, wightened by perturbing representations of clean data via different scales of noise, leveraging the training process of diffusion models. The secondary design is a denoising after diffusion strategy that further brings input noisy data into or close to the noise space modeled by the diffusion models. 
% that first perturbes observed noisy data and then 
% In our method, we learn how to denoise our \rep representations leveraging the training process of diffusion models. 

% Specifically, the diffusion model in our work learns how to project noisy representations from the noise space formed by perturbing the representations via different scales of noise. Given a noisy interaction sequence with novel noise, we further utilize 
% learns how to generate a sequence of

% Instead of learning how to map 
% Gaussian distributio
% any noise to the data manifold. However, it is hard to realize since 
% To address this issue, we devise a denoising strategy based on diffusion models. The core is 

% For instance, the denoising model may only learn how to project the trajectory with Gaussian noise to the corresponding clean sequence. When it is encourntered with another sequence with noise from a completely new distribution, 
% noise-level generalizatin
% in the generalization ability 
% the HOI denoising problem is converted to denoising representations where we c
% Solving the hand-object interaction denoising problem requires us to learn the mapping from noise to data. 

% Specifically, for interaction denoising, we propose a cascaded diffusion strategy to denoise \rep effectively.  It processes the noisy sequence via three sequential denosing modules. Each module cleans one separate part of \rep. 
% We further propose a denoising after diffusion way 
% The denoising projection function is nicely generalizable across different noise distributions taking advantage of 
% % We convert the problem of interaction sequence denoising to representation denoising. 
% Given the above representations extracted from noisy interaction sequence, we then consider to denoise such representations to solve the interaction denoising problem. 
% Considering the complexity of \rep, we design a multi-stage denoising strategy that processes the noisy sequence via three sequential denoising modules. 
% Each denoising module cleans one separate part of such representation. 

% for the interaction denoising. 
% By designing the above representations 
% By converting a hand-object interaction sequence into the above representations, we then convert the problem of interaction denoising into representation denoising. Considering the complexity and the multi-modal information, instead of denoising them together, we propose a multi-stage denoising strategy that denoise each of a separate part of such representation in each stage. 

% The three-stage cascaded denoising is composed of 
% 1) hand motion denoising, where we denoise hand motion trajectories $\{ \mathbf{H}_k \}_{k=1}^K$ with no consideration on object constraints, 2) hand-object spatial denoising, where we denoise the generalized contact-centric hand-object spatial relations to resolve incorrect spatial interaction phenomena such as penetrations, and 3) hand-object temporal denoising, where we denoise the hand-object temporal motion relation representation to induce correct contact and encourage consistent hand-object motions.~\eric{should explain why leveraging a three-stage diffusion. talk about its advantages and comparison with alternatives.}
% At the training time, for each denoising module, we train a diffusion model for its corresponding part of representations based upon ground-truth interaction sequences from the training dataset. When leveraging the diffusion model for sampling, we adopt a denoising after diffusion approach~\ref{fig_method_denoising_after_diffusion}.~\eric{what does this mean? not clear} It first diffuse the representation for a certain number of timesteps. Then the denoising function learned by the diffusion model operates on the diffused representations for denoising. 
% takes the diffused representations 
% For each denoising module, we train a 
% we train a diffusion model for its corresponding part of representations
% % Considering the ambiguity of the denoising task, where we may have multiple reasonable results for one single noisy input, we wish for a generative denoising approach and leverage diffusion models to realize it. 
% Specifically, we devise a diffusion-based paradigm, as illustrated in Figure~\ref{fig_method_denoising_via_diffusion}, and denoise each part of the representation via a diffusion model trained for corresponding representations. 

% For each diffusion model, we need to train a model 
% via a three stage denoising, that is 1) hand motion denoising, where we denoise hand motion trajectories individually without considering constraints imposed by objects, 2) hand-object spatial denoising, where we denoise the generalized contact-centric hand-object spatial relation statistics to resolve unrealistic spatial relations such as penetrations, and 3) hand-object motion denoising, where we denoise the hand-object motion relation representation to induce correct contact and encourage consistent hand-object motions. 

% For each denoising module, we need to train a diffusion model for its corresponding clean representations at realize the denoising process via the denoising via diffusion paradigm. 

% \todo{(the intuition of our method design --- the denoising task is a mapping task in nature, so we should )}

% We leverage diffusion model to perform the denoising task, as illustrated in Figure~\ref{fig_method_denoising_via_diffusion}, to take advantage of its superior ability in depicting a real distribution manifold and learning the noise-to-data mapping in the ambient space. Specifically, we propose a denoising via diffusion paradigm which first diffuse the input representations and denoise the diffused the perturbed noisy data points to a clean data point. 

% (And you should draw to picture to illustrate the basic idea of denoising via diffusion)

% For each denoising module, at the training time, we need to train an individual diffusion model for each kind of representation. Then, at the evaluation stage, where we take a noisy interaction sequence as input and pass it through the three denoising modules sequentially, we denoise the corresponding representations extracted from the input sequence following the denoising via diffusion paradigm. 


\begin{algorithm}[H]
% \algsetup{linenosize=\tiny}
\small 
\caption{\textbf{Denoising via Diffusion}. 
}
\label{algo_denoising_via_diffusion}
\footnotesize
    \begin{algorithmic}[1]
        \Require
            diffusion model $\text{DiffusionModel}=(\text{noise}(\cdot, t), \text{denoise}(\cdot,t))$, input noisy representation $\hat{x}$, diffusion steps $t_\text{diff}$. 
        \Ensure
            denoised data $x$. 

        \Function{Diffuse}{$\hat{x}, t_\text{diff}$} \label{alg:diffuse}

            \For{$t$ from 1 to $t_\text{diff}$}
                \State $\hat{x} \sim \text{noise}(\hat{x}, t)$
            \EndFor
            \\
            \Return $\hat{x}$
        \EndFunction

        \Function{Denoise}{$\hat{x}, t_\text{diff}$}

            \For{$t$ from $t_\text{diff}$ to 1}
                \State $\hat{x} \sim \text{denoise}(\hat{x}, t)$
            \EndFor
            % \State $x\leftarrow \hat{x}$
            \\
            \Return $\hat{x}$
        \EndFunction

        \State $\hat{x} \leftarrow$~\Call{Diffuse}{$\hat{x}, t_\text{diff}$}
        \State $x \leftarrow$~\Call{Denoise}{$\hat{x}, t_\text{diff}$}
        \\
        \Return $x$
    \end{algorithmic}
\end{algorithm}

\noindent \textbf{MotionDiff: canonicalized hand trajectory denoising. 
% Hand motion denoising via diffusion (MotionDiff).
}
This denoising stage removes noise from the canonicalized hand trajectory $\hat{\bar{\mathcal{J}}}$ of the input noisy interaction sequence by applying the diffusion model for motion-denoised $\bar{\mathcal{J}}$, following the denoising via diffusion (Algorithm~\ref{algo_denoising_via_diffusion}) strategy. To do this, the noisy representation $\hat{\bar{\mathcal{J}}}$ is diffused by adding noise for $t_m$ steps, followed by denoising for $t_m$ steps using the diffusion model. The resulting motion-denoised hand trajectory $\mathcal{J}$ in the world coordinate space is obtained by de-canonicalizing the denoised canonicalized hand trajectory $\bar{\mathcal{J}}$ using the pose of the generalized contact points ${ (\mathbf{R}_k, \mathbf{t}_k) }$.
% This denoising stage applies the diffusion model for canonicalized hand trajectories $\bar{\mathcal{J}}$ to remove noise from the canonicalized hand trajectory $\bar{\hat{\mathcal{J}}}$ of the input interaction sequence following the denoising via diffusion (Algorithm~\ref{algo_denoising_via_diffusion}) strategy. The noisy representation $\bar{\hat{\mathcal{J}}}$  is diffused by adding noise for $t_m$ diffusion steps at first. Then, the diffusion model denoises the diffused representation for $t_m$ steps. The motion-denoised hand trajectory  $\mathcal{J}$ can be obtained by utilizing the pose of the generalized contact points $\{ (\mathbf{R}_k, \mathbf{t}_k) \}$ to de-canonicalize the denoised canonicalized hand trajectory $\bar{\mathcal{J}}$. 
% adding the pose of the generalized contact points $\{ (\mathbf{R}_k, \mathbf{t}_k) \}$ back to the denoised canonicalized hand trajectory $\bar{\mathcal{J}}$. 
% For hand motion denoising, the diffusion model is trained on the canonicalized hand trajectories $\mathcal{J}$ from each ground-truth interaction sequence, \emph{i.e.,} $DiffusionModel(\mathcal{J}, t)$. Then, at the test time, we first diffuse the input noisy hand trajectory $\hat{\mathcal{J}}$ for a certain number of steps $t_m$, where $m$ is the indicator for the motion denoising module. Then we utilize the denoising function learned by the denoising model to map the diffused trajectory to the data manifold. We denoted the motion denoised hand trajectory as $\hat{\mathcal{J}}^m$. Formally, 
% \begin{equation}
%     \hat{\mathcal{J}}^m = \text{DENOISE}(\text{DIFFUSE}(\hat{\mathcal{J}}, t_m), t_m). 
% \end{equation}

% \emph{i.e.,}
% $\{  \hat{\mathcal{H}}_k \}_{k=1}^{K}$ by 
% adding $t_m$ steps of noise~\eric{what does $m$ mean here?}, \emph{i.e.,} 
% \begin{equation}
%     \hat{\mathcal{J}}^{t_m} = \text{Diffuse}(\mathcal{J}, t_m).
% \end{equation}
% Then we denoise the perturbed hand trajectory via the trained diffusion model $\epsilon_{\theta_m}(\cdot, \cdot)$ for the motion denoised hand trajectory $\mathcal{J}^m$~\eric{symbols are not consistent with previous ones}. 
% Specifically, we estimate noise $\epsilon_{\theta_m}( \hat{\mathcal{J}}^{t_m} \}_{k=1}^{K}, t )$ of the current trajectory for each denoising time step $t (1 \le t \le t_m)$ via the diffusion model and then sample the trajectory at the previous timestep via the posterior sampling approach, 
% \begin{equation}
%     \{  \mathcal{H}_k^{t-1} \}_{k=1}^{K} = \text{Posterior-Sample} ( \{  \hat{\mathcal{H}}_k^{t} \}_{k=1}^{K}, \epsilon_{\theta_m}( \{  \hat{\mathcal{H}}_k^{t} \}_{k=1}^{K}, t )). 
% \end{equation}
% Finally, we take $\{ \hat{\mathcal{H}}_k^{0} \}_{k=1}^K$  as the motion denoised hand trajectory $\{ \mathcal{H}_k^m \}_{k=1}^K$.
% ~\eric{there are so many subscripts and superscripts, quite annoying and confusing. can we simplify the notation system to reduce their number?}\eric{also the description is not clear enough. I don't understand what you are doing just from what you write down here. What is posterior-sample? is there a reference? also the symbols make me lose track of method flow.}



% $\epsilon_{\theta_m}$ 

% Then we denoise the perturbed hand trajectory via the trained diffusion model to get the denoised hand trajectory $\{  \mathcal{J}_t^m \}_{t=1}^{T}$. 
% the denoised hand trajectory %



\noindent \textbf{SpatialDiff: hand-object spatial denoising.}
The hand-object spatial denoising module operates on the noisy hand-object spatial relations $\hat{\mathcal{S}}$ of the motion-denoised interaction sequence output by the previous MotionDiff stage. The representation $\hat{\mathcal{S}}$  is diffused by adding noise for $t_s$ diffusion steps, followed by another $t_s$ step of denoising. 
% The hand-object spatial denoising module aims to recover the clean hand-object spatial relations $\mathcal{S}$ from motion-denoised hand trajectory with spatial relations $\hat{\mathcal{S}}$. $\hat{\mathcal{S}}$ undergoes $t_s$ diffusion steps, followed by denoising over the same number of steps to obtain the denoised representation $\mathcal{S}$.
% The hand-object spatial denoising module focuses on the hand-object spatial relations $\hat{\mathcal{S}}$ of the motion denoised interaction sequence. Initially, the representation $\hat{\mathcal{S}}$ undergoes $t_s$ diffusion steps. Subsequently, it is denoised back over the $t_s$ steps.
Once we obtain the denoised representation $\mathcal{S}$ which includes the hand-object relative offsets $\{ (\mathbf{h}_k - \mathbf{o}_k) \}$ centered at each generalized contact point $\mathbf{o}_k$, we adopt a simple approach to convert it into a spatial-denoised hand motion sequence. Specifically, we average the denoised hand poses from each object point
% In our method, we adopt a simple approach that employs an averaging operation to combine the denoised results for each object point. Specifically, we compute the average 
as follows:
\begin{equation}
    \mathcal{J} = \text{Average}\{ (\mathbf{h}_k - \mathbf{o}_k ) + \mathbf{o}_k \vert \mathbf{o}_k \in \mathbf{P}_k \}.
    \label{eq_decode_traj_from_spatial}
\end{equation}
% Adding the global pose of generlaized contact points back, we then arrive at the spatial denoised interaction sequence. 
% The spatial denoised interaction sequence 
% is formed by taking the global pose of the generalized contact points and the denoised hand trajectory together. 
% Together with the global pose of the generalized contact points and the spatial denoised trajectory, 
% back to the denoised canonicalized hand trajectory. 
% The denoised canonicalized  trajectory $\mathcal{J}$ 
% we take an easy strategy, 
% The denoising module relies on the diffusion model for the spatial relations $\mathcal{S}$ for denoosing. Then, given $\mathcal{S}^m$, we first diffuse it for a certain steps $t_s$. Then we take the diffusion model to denoise the diffused representation to get the spatial denoised representation $\mathcal{S}^s$, \emph{i.e.,}, 
% \begin{equation}
%     \mathcal{S}^s = \text{DENOISE}(\text{DIFFUSE}(\mathcal{S}^m, t_s), t_s ). 
% \end{equation}
% We can then directly decode the spatial denoised hand trajectory $\mathcal{J}^s$ from the spatial relation representation $\mathcal{S}^s$, \emph{i.e.,}
% \begin{equation}
%     \mathcal{J}^s = \text{Decode}(\mathcal{S}^s). 
% \end{equation}
% Compared with the motion denoised trajectory $\mathcal{J}^m$, $\mathcal{J}^s $ is more object-aware and is expected to be free of penetrations observed in $\mathcal{J}^m$.

% After the hand motion denoising module, we further take constraints imposed by the object into consideration and clean the motion denoised hand trajectory by designing a hand-object spatial denoising module.~\eric{again, please repeat why you cascade a new diffusion model here and why can this step be merged with the previous one.} The spatial denoising module operates on the generalized contact-centric hand-object spatial relations and cleans each relative hand-object position term $\vec{p}_k^h - \vec{p}_k^o$. Specifically, we first train a diffusion model for the representations converted from ground-truth interaction sequences.~\eric{this sentence is weird... what does it mean?} Then, at the test time, we first convert the motion denoised hand trajectory into the corresponding spatial relation representation $\{ \hat{\mathcal{S}}_k \}_[k=1]^K$. We then clean them via the learned denoising function. 

% Specifically, we first perturb the noisy representations $\{ \hat{\mathcal{S}}_k \}_[k=1]^K$ for $t_s$ steps for $\{ \hat{\mathcal{S}}_k^{t_s} \}_{k=1}^K$ following the forward diffusion process. 
% Then we estimate noise of the representation $\{ \hat{\mathcal{S}}_k^{t} \}_[k=1]^K$ at each denoising time step $t (1\le t\le t_s)$ and sample the representation at the previous time step $t-1$~\eric{i know this is standard for diffusion guys but graphics reviewers do not necessarily understand diffusion model. ``previous time step'' sounds like a very strange term in this context. we can refer to some other siggraph journal track papers regarding how to describe this part. some example include ``Blended Latent Diffusion''} via the posterior sampling, \emph{i.e.,}
% \begin{equation}
%     \{ \hat{\mathcal{S}}_k^{t-1} \}_[k=1]^K = \text{Posterior-Sample} ( \{  \hat{\mathcal{S}}_k^{t} \}_{k=1}^{K}, \epsilon_{\theta_s}( \{  \hat{\mathcal{S}}_k^{t} \}_{k=1}^{K}, t )). 
% \end{equation}
% We then take the denoised representation $\{ \hat{\mathcal{S}}_k^{0} \}_[k=1]^K$ at $t=0$ as the denoised spatial representation $\{ {\mathcal{S}}_k \}_{k=1}^K$. 
% After that, we directly decode hand trajectories from the denoised spatial representation by a simple averaging operation, \emph{i.e.,}~\eric{again, avoid using too many superscripts! they introduce confusion! just take $\mathcal{H}_k$ as an example, I have already seen four different superscripts so far.}
% \begin{equation}
%     \{ \mathcal{H}_k^s \}_{k=1}^K = \{ \text{Average}\{ (\vec{p}_k^h - \vec{p}_k^o) + \vec{p}_k^o \vert o\in \mathbf{O}_k \} \}_{k=1}^K. 
% \end{equation}
% hand-object spatial rel
% relative positions 
% relative hand-object positions of the denoised spatial representation via a simple average operation, \emph{i.e.,}
% \begin{equation}
%     \{ \mathcal{H}_k^s \}_{k=1}^K = \{ \text{Average}\{ (\vec{p}_k^h - \vec{p}_k^o) + \vec{p}_k^o \}_{\vec{p}_k^o\in \mathbf{O}_k} \}_{k=1}^K. 
% \end{equation}

% We first train a diffusion model for the
% by leveraging the hand-object 
% we need to further clean the motion denoising trajectory via the spatial denoising module to take objbect 
% leverage the motion denoised hand trajectory $\{ \mathcal{H}_k^m \}_{k=1}^K$ 
% For hand-object spatial relation denoising, we train a diffusion model $\epsilon_{\theta_s}(\cdot, \cdot)$ for the proposed contact-centric hand-object spatial relation representation extracted from clean interaction sequences. 
% Then, at the test time, we first convert the motion denoised interaction sequence into the corresponding spatial relation representation $\{ \hat{\mathcal{S}}_k \}_[k=1]^K$. And they are further cleaned via the denoising via diffusion paradigm via the trained diffusion model on the representation space. 

% Specifically, we first perturb the noisy representations $\{ \hat{\mathcal{S}}_k \}_[k=1]^K$ for $t_s$ steps for $\{ \hat{\mathcal{S}}_k^{t_s} \}_{k=1}^K$ following the forward diffusion process. 
% Then we estimate noise of the representation $\{ \hat{\mathcal{S}}_k^{t} \}_[k=1]^K$ at each denoising time step $t (1\le t\le t_s)$ and sample the representation at the previous time step $t-1$ via the posterior sampling, \emph{i.e.,}
% \begin{equation}
%     \{ \hat{\mathcal{S}}_k^{t-1} \}_[k=1]^K = \text{Posterior-Sample} ( \{  \hat{\mathcal{S}}_k^{t} \}_{k=1}^{K}, \epsilon_{\theta_s}( \{  \hat{\mathcal{S}}_k^{t} \}_{k=1}^{K}, t )). 
% \end{equation}
% We then take the denoised representation $\{ \hat{\mathcal{S}}_k^{0} \}_[k=1]^K$ at $t=0$ as the denoised spatial representation $\{ {\mathcal{S}}_k \}_{k=1}^K$. 
% After that, we directly decode hand trajectories from relative hand-object positions of the denoised spatial representation via a simple average operation, \emph{i.e.,}
% \begin{equation}
%     \{ \mathcal{H}_k^s \}_{k=1}^K = \{ \text{Average}\{ (\vec{p}_k^h - \vec{p}_k^o) + \vec{p}_k^o \}_{\vec{p}_k^o\in \mathbf{O}_k} \}_{k=1}^K. 
% \end{equation}

% primal representation space leveraging the standard DDPM process. 
% % on the primal
% Then, at the test time, we first convert the motion denoised hand trajectory and the object sequence into the corresponding spatial relation representation. They are further cleaned via the denoising via diffusion paradigm together with the trained diffusion model on the representation space. 
% use a denoised motion trajectory from we can directly
% We can directly decode a hand-object spatial relation denoised motion trajectory from the denoised relation-related representation. We simply use an average operation to realize it (TODO: add a formula). Next, we extract hand-object motion-related representation from the relation denoised motion trajectory and the object sequence. We denote it as xxx. 

\noindent \textbf{TemporalDiff: hand-object temporal denoising.}
% After the motion denoising and the spatial denoising, we then need to further clean the hand-object temporal relations $\hat{\mathcal{T}}$ of the spatial denoised sequence to remove temporal noise. The temporal motion relations are also cleaned following the denoising via deiffusion procedure. 
% After that, to get the temporal denoised hand trajectory, we add an optimization step that optimizes the spatial denoised interaction sequence so that the hand-object temporal motion relations $\mathcal{T}^s$ is close to the denoised relations $\mathcal{T}$. 
% The objective is as follows:
% \begin{equation}
%     \text{minimize}\Vert \mathcal{T}^s - \mathcal{T} \Vert,
% \end{equation}
% where the distance is calculated on two relative velocity related statistics, \emph{i.e.,} $\{ e_{k,\parallel}^{\mathbf{ho}}, e_{k,\perp}^{\mathbf{ho}} \}$. We simply leverage an AdaM optimizer to find the optimal hand trajectory. The optimized trajectory is take as the final denoised trajectory $\mathcal{J}$. 
Following MotionDiff and SpatialDiff, we proceed to clean the noisy hand-object temporal relations $\hat{\mathcal{T}}$ of the spatial-denoised sequence.
% the in order to eliminate temporal noise.
The denoising via diffusion procedure is applied to the temporal motion relations to achieve this. The temporal relations cannot be converted to the hand trajectory directly like what we do for the spatial representation (Equation~\ref{eq_decode_traj_from_spatial}). Thus, to obtain the temporal-denoised hand trajectory, an additional optimization step is introduced. 
% The denoised temporal representations cannot be converted to the denoised hand 
% To obtain the temporal-denoised hand trajectory, an additional optimization step is introduced. 
This optimization step aims to refine the spatial-denoised sequence so that its hand-object temporal motion relations $\hat{\mathcal{T}}$ closely match the denoised relations $\mathcal{T}$. The objective of the optimization is formulated as follows:
\begin{equation}
    \underset{\hat{\mathcal{T}}}{\text{minimize}}\Vert \hat{\mathcal{T}} - \mathcal{T} \Vert,
    \label{eq_optimization_temporal}
\end{equation}
where the objective is calculated on hand-object distances, \emph{i.e.,} $\{ d_k^{\mathbf{ho}} \}$, and two relative velocity-related statistics ( $\{ e_{k,\parallel}^{\mathbf{ho}}, e_{k,\perp}^{\mathbf{ho}} \}$ ). We employ an AdaM optimizer to find the optimal hand trajectory. The optimized trajectory is taken as the final denoised trajectory $\mathcal{J}$. 
% \eric{Please explain why this optimization is necessary.}


% that 
% optimizes from the spatial denoised trajectory $\mathcal{J}^s$ to minimize the distance between the temporal 
% we add an optimization step that 
% that utilizes the two kinds of denoised relative velocity related statistics $\{ (e_{k,\parallel}^{\mathbf{ho}}, e_{k,\perp}^{\mathbf{ho}}) \}$ from the denoised temporal relations $\mathcal{T}$ to optimize the spatial denoised hand trajectory. 

% \emph{i.e.,}
% \begin{equation}
%     \mathcal{J} = \text{argmin}_{\mathcal{J}}\Vert \mathcal{T}(\mathcal{J}) -  \Vert
%     \mathcal{J} = \text{Optimize}(\mathcal{J}^s, \mathcal{T}, \mathcal{P}). 
% \end{equation}
% $\mathcal{P}$ is the trajectory of generalized contact points. 

% At the test time, we first induce the noisy temporal hand-object motion relations $\{ \hat{\mathcal{T}}_k \}_[k=1]^{K-1}$  from the spatial denoised hand trajectory $\mathcal{H}$. Then we first diffuse the noisy representation $\{ \hat{\mathcal{T}}_k \}_[k=1]^K$ for $t_t$ steps, resulting in $\{ \hat{\mathcal{T}}_k^{t_t} \}_{k=1}^{K-1}$.~\eric{I remember you are using latent diffusion for this step? The three diffusion does not seem to differ much and the writing does not convey any insights about this cascaded diffusion process} Then the diffusion model is leveraged to denoise the perturbed representation for $t_t$ steps for the cleaned representation, \emph{i.e.,}  $\{ {\mathcal{T}}_k \}_{k=1}^{K-1}$. We then refine the spatial denoised hand trajectory via the denoised energies
% ~\eric{what does this energy term mean? The optimization step seems to be important but obtains short shrift.} 
% $\{  ( e_{k, \parallel}^{ho}, e_{k, \perp}^{ho} ) \vert o \in \mathbf{O}, h \in \mathbf{H} \}$. It is completed by an optimization step, where we optimize the hand trajectory $\{ \mathbf{H}_k \}$ so that the energies induced by the optimized trajectory are close to the denoised energies. We use an AdaM optimizer to solve the optimization problem. 

% the spatial denoising and 
% The hand-object temporal denoising module operates on the temporal hand-object motion relation representation of the interaction sequence cleaned via the first two denoising modules. 
% By first perturbing the noisy representation $\{ \hat{\mathcal{T}}_k \}_[k=1]^K$ for $t_t$ steps, resulting $\{ \hat{\mathcal{T}}_k^{t_t} \}_{k=1}^K$ following the forward diffusion process. 
% Then we denoise the perturbed representation via the trained diffusion model for $t_t$ steps for the cleaned representation, \emph{i.e.,}  $\{ {\mathcal{T}}_k \}_{k=1}^K$. 
% We then refine the hand motion trajectory denoised by the first two modules via the denoised energies $\{  e_{k, \parallel}^{ho} \vert \vec{p}_k^o \in \mathbf{O}_k, \vec{p}_k^h\in \mathbf{J}_k \}$. 
% It is processed by an optimization step, where we optimize the hand trajectory $\{ \mathbf{J}_k \}$ so that the energies induced by the optimized trajectory are close to the denoised energies. 
% We simply use an AdaM optimizer to realize the optimization. 

\subsection{Fitting for a Hand-Object Interaction Trajectory}
% After we have denoised the interaction sequence via the above three denoising modules, we need to further fit a sequence of hand parametric models, MANO~\cite{romero2022embodied} model, for final hand meshes. 
% Specifically, we need to optimize a series of hand MANO parameters $\{\mathbf{r}_k, \mathbf{t}_k, \mathbf{\beta}_k, \mathbf{\theta}_k\}_{k=1}^K$ to reconstruct the prediction, such that the hand trajectory representation $\mathcal{J}^{recon}$ are close to the denoised trajectory $\mathcal{J}$. Since the hand trajectory $\mathcal{J}$ contains the sequence of hand keypoints, a subset of hand mesh vertices, the reconstruction is also added on such keypoints. The process of deriving keypoints from MANO parameters is differentiable. Therefore the reconstruction can optimize the MANO parametes finally. 
% Specifically, we leverage an AdaM optimizer to minimize the reconstruction loss 
% \begin{equation}
%     \mathcal{L}_{recon} = \Vert \mathcal{J} - \mathcal{J}^{recon} \Vert. 
% \end{equation}
% The distance function is a simple MSE between the hand keypoints at each frame. We further add regularization losses to regularize hand parameters $\{ \mathbf{\beta}_k, \mathbf{\theta}_k \}$ and their temporal smoothness. Specifically, the regularization loss is as follows, 
% \begin{equation}
%     \mathcal{L}_{reg} = \frac{1}{K} \sum_{k=1}^{K}( \Vert \mathbf{\beta}_k \Vert_2 + \Vert \mathbf{\theta}_k \Vert_2 ) + \frac{1}{K-1} \sum_{k=1}^{K-1}\Vert \mathbf{\theta}_{k+1} - \mathbf{\theta}_k \Vert_2. 
% \end{equation}
% The optimization objective is formalized as, 
% \begin{equation}
%     \text{minimize}_{\{ \mathbf{r}_k, \mathbf{t}_k, \mathbf{\beta}_k, \mathbf{\theta}_k \}_{k=1}^K} (\mathcal{L}_{recon} + \mathcal{L}_{reg}). 
%     \label{eq_optimization}
% \end{equation}
% We use an Adam optimizer to solve the fitting problem. 

Once the interaction sequence has been denoised via the above denoising modules, we proceed to fit a sequence of hand parametric models, specifically the MANO model~\cite{romero2022embodied}, to obtain the final hand meshes.
The objective is to optimize a series of MANO hand parameters $\{ \mathbf{r}_k, \mathbf{t}_k, \mathbf{\beta}_k, \mathbf{\theta}_k \}_{k=1}^K$ so that they fit the denoised trajectory $\mathcal{J}$ well. Notice the hand trajectory $\mathcal{J}$ consists of a sequence of hand keypoints so we also need to derive keypoints from MANO parameters to allow the above optimization. Luckily this process is differentiable and we use $\mathcal{J}^{recon}(\{ \mathbf{r}_k, \mathbf{t}_k, \mathbf{\beta}_k, \mathbf{\theta}_k \}_{k=1}^K)$ to denote it. 
% in order to reconstruct the prediction, such that the hand trajectory representation $\mathcal{J}^{recon}$ closely matches the denoised trajectory $\mathcal{J}$. Since the hand trajectory $\mathcal{J}$ consists of a sequence of hand keypoints, which are a subset of the hand mesh vertices, the reconstruction process involves optimizing these keypoints. The process of deriving keypoints from MANO parameters is differentiable, allowing us to optimize the MANO parameters accordingly.
We can therefore optimize the following reconstruction loss for the MANO hands
\begin{equation}
    \mathcal{L}_{recon} = \Vert \mathcal{J} - \mathcal{J}^{recon}(\{ \mathbf{r}_k, \mathbf{t}_k, \mathbf{\beta}_k, \mathbf{\theta}_k \}_{k=1}^K) \Vert,
    \label{eq_recon_losses}
\end{equation}
where the distance function is a simple mean squared error (MSE) between the hand keypoints at each frame. To regularize the hand parameters $\{ \mathbf{\beta}_k, \mathbf{\theta}_k \}$ and enforce temporal smoothness, we introduce an additional regularization loss defined as
\begin{equation}
    \mathcal{L}_{reg} = \frac{1}{K} \sum_{k=1}^{K}( \Vert \mathbf{\beta}_k \Vert_2 + \Vert \mathbf{\theta}_k \Vert_2 ) + \frac{1}{K-1} \sum_{k=1}^{K-1}\Vert \mathbf{\theta}_{k+1} - \mathbf{\theta}_k \Vert_2. 
    \label{eq_reg_fitting}
\end{equation}
The overall optimization objective is formalized as
\begin{equation}
    \text{minimize}_{\{ \mathbf{r}_k, \mathbf{t}_k, \mathbf{\beta}_k, \mathbf{\theta}_k \}_{k=1}^K} (\mathcal{L}_{recon} + \mathcal{L}_{reg}), 
    \label{eq_optimization}
\end{equation}
and we employ an AdaM optimizer to solve the fitting problem.
% and a series of regularization losses such as pose prior loss.~\eric{too sketchy...} The optimization problem is formalized as: 

% ~\eric{please remind the reader what the keypoints mean. the easier way is to connect $\{ \mathbf{H}_k \}$ with keypoints at the beginning of the paragraph.} 

% a suit of hand MANO parameters such that hand keypoints are consistent with the denoised trajectory. 
% \todo{The fitting process here}

% For the hand-object motion denoising module, we first train a diffusion model for such representation leveraging the latent diffusion paradigm. 
% The diffusion model is then further leveraged to clean the above extracted representations to get the denoised hand-object motion relations. Based on the denoised representation, we add an optimization stage to correct the relation denoised hand trajectory output from the second stage. 


% \todo{(TODO: we think we need to make the intuition under the method clearer to make it easy to understand)}







==> articles/repro_statement.tex <==
\section{Reproducibility Statement}

\noindent \textbf{Novel Models and Algorithms.}
Our method is composed of two novel designs: 
1) The \rep representation. We have provided detailed explanations of the representation in Section~\ref{sec:geneoh} and Appendix~\ref{sec_appen_rep_design}. Besides, we have included the source code in the Supplementary Materials, where the implementations of \rep are contained. Please refer to \emph{Key Implementations} section in the file \emph{Geneoh-Diffusion-Code/README.md} in our Supplementary Materials. 
2) The progressive HOI denoising method. We have provided detailed explanations of the denoising method in Section~\ref{sec:diffusion} and Appendix~\ref{sec_genenoh_diffusion_details}. Model, training, and evaluation details are included in Appendix~\ref{sec_appen_model_details} and~\ref{sec_appen_training_details}. Besides, we have included the source code in the Supplementary Materials. Please refer to the \emph{Key Implementations} section and \emph{Usage} section in the file \emph{Geneoh-Diffusion-Code/README.md} in our Supplementary Materials. 

\noindent \textbf{Theoretical Results.}
Please refer to section~\ref{sec_appen_rep_design} in the Appendix for the proof of the property of leveraging the stage-wise denoising can clean the noisy input where each stage would not comprise the naturalness achieved after previous denoising stages. 

\noindent \textbf{Datasets.}
Please refer to Section~\ref{sec_exp_settings} and Appendix~\ref{sec_appen_datasets} for a detailed explanation of the datasets used. The data preprocessing part can be found in the \emph{Data Preprocessing} section in the file \emph{Geneoh-Diffusion-Code/README.md} in our Supplementary Materials. 

\noindent \textbf{Experiments.} 
For experiments, we provide 1) Source code.
% of our implementation. 
Please refer to the folder \emph{Geneoh-Diffusion-Code} in our Supplementary Materials for details. 
2) Experimental details of our method and compared baselines. Please refer to the Section~\ref{sec_exp_settings} and in the Appendix~\ref{sec_exp_details} for details. 
We also provide related information and instructions in the \emph{Geneoh-Diffusion-Code/README.md} file. 


==> guide.tex <==




\section{Submission of conference papers to ICLR 2024}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2024 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2024_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2024_conference.sty+ and \verb+iclr2024_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2024_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.


\bibliography{ref}
\bibliographystyle{iclr2024_conference}

\appendix
\section{Appendix}
You may include other additional sections here.


